McFly: Time-Travel Debugging for the Web

Time-traveling debuggers offer the promise of simplifying debugging by letting developers freely step forwards and backwards through a program's execution. However, web applications present multiple challenges that make time-travel debugging especially difficult. A time-traveling debugger for web applications must accurately reproduce all network interactions, asynchronous events, and visual states observed during the original execution, both while stepping forwards and backwards. This must all be done in the context of a complex and highly multithreaded browser runtime. At the same time, to be practical, a time-traveling debugger must maintain interactive speeds. This paper presents McFly, the first time-traveling debugger for web applications. McFly departs from previous approaches by operating on a high-level representation of the browser's internal state. This approach lets McFly provide accurate time-travel debugging - maintaining JavaScript and visual state in sync at all times - at interactive speeds. McFly's architecture is browser-agnostic, building on web standards supported by all major browsers. We have implemented McFly as an extension to the Microsoft Edge web browser, and core parts of McFly have been integrated into a time-traveling debugger product from Microsoft.

==> Makefile <==
MAIN = main

PDFLATEX = pdflatex -halt-on-error -interaction nonstopmode -shell-escape
BIBTEX = bibtex
PATCH = patch -p0 -t

R ?= HEAD
DIFF_DIR = .diff.$(R)
OLDVERSION_DIR = .oldversion.$(R)
CHANGES_FILE = .changes.$(R).diff

SIDE_EFFECTS = $(MAIN).pdf $(MAIN).out $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log diff.pdf \
	$(wildcard diff.*) $(wildcard oldversion.*) $(wildcard changes.*)

FILES = $(filter-out $(SIDE_EFFECTS), $(wildcard *))
TEX_FILES = $(wildcard *.tex)
NONTEX_FILES = $(filter-out $(TEX_FILES), $(FILES))

OLD_FILES = $(addprefix $(OLDVERSION_DIR)/, $(FILES))
OLD_TEX_FILES = $(addprefix $(OLDVERSION_DIR/, $(TEX_FILES))
OLD_NONTEX_FILES = $(addprefix $(OLDVERSION_DIR/, $(NONTEX_FILES))

DIFF_FILES = $(addprefix $(DIFF_DIR)/, $(FILES))
DIFF_TEX_FILES = $(addprefix $(DIFF_DIR)/, $(TEX_FILES))
DIFF_NONTEX_FILES = $(addprefix $(DIFF_DIR)/, $(NONTEX_FILES))

all: $(MAIN).pdf $(MAIN).bbl

clean:
	@rm -f $(MAIN).pdf $(MAIN).out $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log
	@rm -rf diff.pdf .oldversion.* .diff.* .changes.*

$(MAIN).pdf: $(wildcard *.tex)
	@echo "[MAIN] Running pdflatex"
	@$(PDFLATEX) $(MAIN).tex | tail

$(MAIN).bbl: $(wildcard *.bib)
	@echo "[MAIN] Running bibtex"
	@$(BIBTEX) $(MAIN).aux

	@echo "[MAIN] Updating document references"
	@$(PDFLATEX) $(MAIN).tex > /dev/null
	@$(PDFLATEX) $(MAIN).tex > /dev/null

diff: diff.pdf

diff.pdf: $(DIFF_DIR)/$(MAIN).pdf $(DIFF_DIR)/$(MAIN).bbl
	@cp $(DIFF_DIR)/$(MAIN).pdf diff.pdf

$(DIFF_DIR)/$(MAIN).pdf: $(DIFF_NONTEX_FILES) $(DIFF_DIR)/$(MAIN).tex
	@echo "[DIFF] Running pdflatex"
	@cd $(DIFF_DIR); $(PDFLATEX) $(MAIN).tex | tail

$(DIFF_DIR)/$(MAIN).bbl: $(wildcard $(DIFF_DIR)/*.bib)
	@echo "[DIFF] Running bibtex"
	@cd $(DIFF_DIR); $(BIBTEX) $(MAIN).aux
	@echo "[DIFF] Updating document references"
	@cd $(DIFF_DIR); $(PDFLATEX) $(MAIN).tex > /dev/null
	@cd $(DIFF_DIR); $(PDFLATEX) $(MAIN).tex > /dev/null

$(DIFF_DIR)/$(MAIN).tex: oldversion_dummy
	@echo "[DIFF] Running latexdiff"
	@mkdir -p $(DIFF_DIR)
	@latexdiff --flatten $(OLDVERSION_DIR)/$(MAIN).tex $(MAIN).tex > $@ 2> /dev/null

$(DIFF_NONTEX_FILES): oldversion_dummy
	@echo "[DIFF] Copying $(notdir $@) to diff workspace"
	@mkdir -p $(DIFF_DIR)
	@cp -R $(notdir $@) $@

oldversion_dummy: $(CHANGES_FILE)
	@echo "[DIFF] Copying files to old version workspace"
	@mkdir -p $(OLDVERSION_DIR)
	@cp -R $(FILES) $(OLDVERSION_DIR)/
	@echo "[DIFF] Applying changes to old version workspace"
	@$(PATCH) -R -d $(OLDVERSION_DIR) -i ../$(CHANGES_FILE)

$(CHANGES_FILE): $(FILES)
ifeq ($(R),HEAD)
	@echo "[DIFF] Using local checkout to compute changes"
	@git diff *.tex > $@
else
	@echo "[DIFF] Fetching changes from repository"
	@git diff -r $(R):HEAD > $@
endif


==> discussion.tex <==
% !TeX root = main.tex
\section{Discussion}
\label{sec:discussion}

We believe that the interrogative interfaces described in Section~\ref{sec:mechanisms} are portable to other browsers, and can be re-purposed to enable efficient program migration across the network.
We discuss both of these ideas below.

\point{Portability to other browsers:} We implemented \sys and our interrogative interfaces in a single web browser.
The architecture of most web browsers closely mirror Figure~\ref{fig:browser-arch}; they have separate JavaScript and rendering engines (V8/Blink, SpiderMonkey/Gecko, Chakra/Edge), dedicated I/O and animation threads or processes, and their rendering engines expose the same standard JavaScript interfaces described in \autoref{fig:state-table}.
We believe that the engineering effort required to port ReJS is modest.
Porting would require re-implementing our interrogative interfaces (\S\ref{sec:js-proto}), JavaScript heap serialization/deserialization (\S\ref{subsec:checkpoints}), and performance monitoring (\S\ref{subsec:perf-monitoring}).

\point{Program migration:} Interrogative interfaces let \sys accurately capture a web application's entire state into checkpoints, which is also useful for live program migration.
Initial experiments show that \sys can use its efficient checkpoint primitives to live migrate our benchmark applications between computers \emph{within a second} on a 10Mbps connection.
%Live migration only requires one extra interrogative interface to capture pending JavaScript events.
Live migration required a trivial set of changes to checkpoint logic; for example, network connections must emit the proper JavaScript events to migrate to an \emph{error} state to emulate network downtime, and pending timers must be allowed to fire naturally.


